VisGym: Diverse, Customizable, Scalable Environments for Multimodal Agents

Modern Vision-Language Models (VLMs) remain poorly characterized in multi-step visual interactions, particularly in how they integrate perception, memory, and action over long horizons. We introduce VisGym, a gymnasium of 17 environments for evaluating and training VLMs. The suite spans symbolic puzzles, real-image understanding, navigation, and manipulation, and provides flexible controls over difficulty, input representation, planning horizon, and feedback. We also provide multi-step solvers that generate structured demonstrations, enabling supervised finetuning. Our evaluations show that all frontier models struggle in interactive settings, achieving low success rates in both the easy (46.6%) and hard (26.0%) configurations. Our experiments reveal notable limitations: models struggle to effectively leverage long context, performing worse with an unbounded history than with truncated windows. Furthermore, we find that several text-based symbolic tasks become substantially harder once rendered visually. However, explicit goal observations, textual feedback, and exploratory demonstrations in partially observable or unknown-dynamics settings for supervised finetuning yield consistent gains, highlighting concrete failure modes and pathways for improving multi-step visual decision-making. Code, data, and models can be found at: https://visgym.github.io/.

==> math_commands.tex <==

\usepackage{amsmath,amsfonts,bm}

\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

\newcommand{\newterm}[1]{{\bf #1}}


\def\figref#1{figure~\ref{#1}}
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
\def\secref#1{section~\ref{#1}}
\def\Secref#1{Section~\ref{#1}}
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
\def\eqref#1{equation~\ref{#1}}
\def\Eqref#1{Equation~\ref{#1}}
\def\plaineqref#1{\ref{#1}}
\def\chapref#1{chapter~\ref{#1}}
\def\Chapref#1{Chapter~\ref{#1}}
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
\def\algref#1{algorithm~\ref{#1}}
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
\def\partref#1{part~\ref{#1}}
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{p_{\rm{data}}}
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} %

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sec/0_abstract.tex <==
\begin{abstract}


\noindent Modern Vision–Language Models (VLMs) remain poorly characterized in multi-step visual interactions, particularly in how they integrate perception, memory, and action over long horizons.
We introduce \ours{}, a gymnasium of $17$ environments for evaluating and training VLMs.  
The suite spans symbolic puzzles, real-image understanding, navigation, and manipulation, and provides flexible controls over difficulty, input representation, planning horizon, and feedback.  
We also provide multi-step solvers that generate structured demonstrations, enabling supervised finetuning.
Our evaluations show that all frontier models struggle in interactive settings, achieving low success rates in both the easy ($46.6\%$) and hard ($26.0\%$) configurations.
Our experiments reveal notable limitations: models struggle to effectively leverage long context, performing worse with an unbounded history than with truncated windows. Furthermore, we find that several text-based symbolic tasks become substantially harder once rendered visually.
However, explicit goal observations, textual feedback, and exploratory demonstrations in partially observable or unknown-dynamics settings for supervised finetuning yield consistent gains, highlighting concrete failure modes and pathways for improving multi-step visual decision-making.
Code, data, and models can be found at: \href{https://visgym.github.io/}{\underline{VisGym.github.io}}. \\[0.5em]
\noindent\small\textbf{Correspondence:}\;
\texttt{%
\{}%
\href{mailto:zwcolin@eecs.berkeley.edu}{\texttt{zwcolin}}%
\texttt{,}%
\href{mailto:junyizhang@eecs.berkeley.edu}{\texttt{junyizhang}}%
\texttt{,}%
\href{mailto:gejiaxin@eecs.berkeley.edu}{\texttt{gejiaxin}}%
\texttt{\}@eecs.berkeley.edu}%
\\[0.2em]


\end{abstract}














==> sec/1_intro_colm.tex <==


\vspace{-9.5ex}
\begin{figure}[h]
    \centering
    \includegraphics[width=0.995\linewidth]{figures/teaser.pdf}
    \vspace{-2ex}
    \caption{\textbf{An overview of \ours.} (\textit{Left}) \ours{} consists of $17$ diverse, long-horizon environments designed to systematically evaluate, diagnose, and train VLMs on visually interactive tasks with different domains, levels of state observability, and types of observations. (\textit{Right}) An example trajectory for the Maze 3D navigation task illustrates a partially observable environment consisting of non-structured synthetic renderings. Here, a VLM is prompted with (1) the task description (\textit{simplified in the figure}) and (2) a set of available actions to use (\textit{not shown in the figure for simplicity}). The agent must select each action conditioned on both its past actions and observation history for its decision-making. \colin{change h and t}}
    \label{fig:teaser}
\end{figure}

\section{Introduction}
\label{sec:intro}

Humans navigate complex tasks in visually rich and interactive settings: manipulating objects, using devices, or exploring unfamiliar environments.
Success in these settings hinges on the tight coupling of perception, memory, and action over multiple steps \citep{Gibson1979TheEA, Henderson2001ASA}.
Foundation Vision–Language Models (VLMs) have made remarkable progress on static vision–language benchmarks
\citep{yue2024mmmu, lu2023mathvista, wang2024charxiv}
and on text-based multi-step tasks such as web browsing and coding
\citep{sirdeshmukh2025multichallenge, wei2025browsecomp, jimenez2023swe}.
Yet when visual observations must be integrated into multi-step decision-making, their behavior remains far less understood.
Recent evaluations across robotic manipulation, computer-use agents, and gaming agents highlight a range of challenges for visually interactive decision-making, including low task success rates, brittle visual grounding, and weak generalization \citep{zhang2025vlabench, xie2024osworld, zhang2025videogamebench, liu2023libero, hu2025lmgame, chen2025g1, shi2025korgym, liu2024visualagentbench}.
Although these insights are valuable, they tend to be domain-specific and observational, offering limited \emph{systematic, controlled} diagnosis of how domain-agnostic factors—such as context length, representation modality, feedback design, or goal visibility—affect model performance across tasks.

We introduce \ours{}, a highly diverse, scalable, and customizable gymnasium with 17 long-horizon environments designed to isolate what limits interactive decision-making across domains and to expose where current VLMs break down.
The suite spans symbolic puzzles, real-image understanding, navigation, and manipulation tasks, each with distinct observability and dynamics and equipped with oracle multi-step solvers for supervised finetuning (framework comparison in \cref{tab:framework_comparisons}).
Crucially, \ours{} provides fine-grained controls over input representation, difficulty, history length, planning horizon, and feedback, enabling domain-agnostic, systematic analysis of model behavior.
Building on prior domain-specific studies, we conduct cross-domain controlled experiments that examine how these factors, together with module finetuning and data curation, affect performance in multi-step visual decision-making.

Across $11$ state-of-the-art models, even the strongest achieve only $26.79\%$ and $12.57\%$ success in the easy and hard settings, respectively.
Our analyses reveal several concrete, cross-domain failure modes: 
\textbf{\textit{(1)}} models struggle to effectively leverage long-term context, showing a reversed-U relationship where performance degrades as the context grows unbounded; \textbf{\textit{(2)}} VLMs struggle with low-level perceptual grounding, a limitation highlighted by symbolic variants of tasks being substantially easier than their visually rendered counterparts; \textbf{\textit{(3)}} models struggle to infer task states and outcomes from purely visual transitions, consistently relying on explicit textual feedback to boost performance; \textbf{\textit{(4)}} the benefit of providing explicit goal observations is brittle and can backfire: while explicit goals can yield large gains, limited visual perception can cause models to misidentify them and, paradoxically, perform worse than with no goal at all; \textbf{\textit{(5)}} models fail to learn from standard demonstrations under partial observability or unknown dynamics, requiring information-revealing demonstrations that expose hidden states or clarify dynamics to significantly improve supervised finetuning outcomes.

Together, these findings establish \ours{} as a unified and extensible framework for diagnosing, understanding, and ultimately improving VLMs in visually interactive decision-making.



\input{tables/framework_comparisons}


























==> sec/5_training_colm.tex <==
\section{Training with \ours}
\label{sec:train}

We describe our supervised fine-tuning experiments with \ours{}, present results, and provide insights on generalization, module specificity, and data curation.

\subsection{Supervised Fine-Tuning Experiments}
\label{subsec:sft_exp}

\myparagraph{Setup.}
We generate demonstration trajectories for supervised fine-tuning using the multi-step solver described in \cref{para:solver}.
We apply two preprocessing filters: (1) discarding trajectories that fail to complete the task, and (2) removing trajectories with initial states overlapping the test split to prevent data leakage.

We evaluate two fine-tuning configurations: \textit{single-task} and \textit{mixed-task}.
In the \textit{single-task} setting, we fine-tune a separate model for each task, whereas in the \textit{mixed-task} setting, a single model is trained jointly on all tasks.
Notably, demonstrations are sourced exclusively from the easy difficulty level; thus, performance on the hard setting serves as a metric for difficulty generalization.
All experiments employ Qwen2.5-VL-7B-Instruct~\citep{bai2025qwen2} with full-parameter fine-tuning, a global batch size of $64$, a learning rate of $1 \times 10^{-5}$, and \texttt{bf16} precision.
Models are trained for $1,500$ steps in the single-task setting and $5,000$ steps in the mixed-task setting.
We utilize LlamaFactory~\citep{zheng2024llamafactory} for all data preprocessing and training orchestration.

\myparagraph{Results.} 
As shown in \cref{fig:main_result,fig:main_result_avg}, finetuned models achieve state-of-the-art performance on most tasks, validating both the learnability of our environments and the effectiveness of our multi-step solvers.  
These gains confirm that current VLMs can substantially benefit from structured, solver-generated demonstrations in visually grounded multi-step settings.



\subsection{Stronger Base Model Generalizes Better}
\label{subsec:base_generalization}
\input{figs/train_variant_generalization}
Existing work has discussed the limitations of supervised finetuning \citep{ross2011reduction} and found that it exhibits limited generalization to task variants \citep{caccia2024finetuning, deng2023mind2web, jang2022bc}.  
This motivates re-examining generalization in the context of modern VLMs, whose capabilities may shift the boundary of what supervised finetuning can or cannot retain.

To this end, we select a set of environments where the easy-to-hard difficulty gap introduces substantial state changes (\textit{e.g.}, more views in the Zoom-In Puzzle, more patches in Patch Reassembly, larger maze sizes; details in \cref{appx:task_variant_generalization}).  
We finetune Qwen2.5-VL-7B-Instruct and Qwen3-VL-8B-Instruct on the same mixed-task training data using identical optimization hyperparameters (see \cref{subsec:sft_exp}), and report performance in \cref{fig:train_variant_gen}.

As shown, both models achieve comparable performance on the easy variants they were trained on (\textit{e.g.}, $0.59$ vs.\ $0.64$), but the more recent Qwen3-VL generalizes substantially better to the harder variants, nearly doubling the success rate on average relative to Qwen2.5-VL.
This trend highlights that newer VLMs provide stronger out-of-distribution generalization in multi-step visual decision-making despite being finetuned on an identical setup.


\subsection{Vision and LLM Both Matter}
\input{figs/train_modules}
Classic perception–action theories emphasize that fine-grained visual encoding and temporal integration are jointly necessary for interactive behavior \citep{Gibson1979TheEA}.  
We examine whether this holds for VLMs by fine-tuning variants that modify either the vision encoder or the LLM backbone to isolate each module’s contribution, where the vision encoder provides fine-grained perceptual features and the LLM performs temporal integration across steps.  

As shown in \cref{fig:train_modules}, most tasks benefit from fine-tuning both components, with the LLM contributing the larger performance gain—particularly in tasks with partial observability or unknown environment dynamics.  
This highlights that temporal reasoning and history integration remain the primary bottlenecks for current VLMs, while strong fine-grained visual encoding is necessary (\textit{e.g.,} Zoom-In Puzzle primarily benefits from vision finetuning) but often not sufficient for multi-step decision-making.





